Learning an Unreferenced Metric for Online Dialogue Evaluation

Evaluating the quality of a dialogue interaction between two agents is a difficult task, especially in open-domain chit-chat style dialogue. There have been recent efforts to develop automatic dialogue evaluation metrics, but most of them do not generalize to unseen datasets and/or need a human-generated reference response during inference, making it infeasible for online evaluation. Here, we propose an unreferenced automated evaluation metric that uses large pre-trained language models to extract latent representations of utterances, and leverages the temporal transitions that exist between them. We show that our model achieves higher correlation with human annotations in an online setting, while not requiring true responses for comparison during inference.

==> Unref Dialog Eval - ACL/figures/human_uncalib.tex <==
\begin{figure}[!htb]
     \centering
    \includegraphics[width=0.5\textwidth]{figures/plot_2.png}
    \caption{\small{Human correlation on un-calibrated scores collected on PersonaChat dataset \cite{zhang2018personalizing}, for \dtm{}, DistilBERT-NLI, InferSent and RUBER}}
    \label{fig:human_corr}
\end{figure}

==> Unref Dialog Eval - ACL/figures/model_diagram.tex <==
\begin{figure}[htb]
\centering
%\resizebox{0.5\textwidth}{!}{\includegraphics[]{figures/model_diag_desc.jpeg}}
%\resizebox{0.5\textwidth}{!}{\input{figures/model_diagram.tikz}}
\caption{Model diagram of \dtm{}}\label{fig:model_diagram}
\end{figure}

==> Unref Dialog Eval - ACL/figures/temporal_structure_two.tex <==
\begin{figure}[!htb]
     \centering
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/frames_short.png}}}%
    \qquad
    \hspace{-27pt}
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/LDA_personachat_finetuned.png}}}%
    \caption{LDA downsampled representation of BERT on Frames (Goal oriented), and PersonaChat (chit-chat). The clusters denote the binning of each utterance, where purple denotes the first bin and red denotes the last bin.}
    \vspace{-10pt}
    \label{fig:dialog_structure_small}
\end{figure}

==> Unref Dialog Eval - ACL/figures/temporal_structures.tex <==
\begin{figure*}[h]
     \centering
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/frames_short.png}}}%
    \qquad
    \hspace{-20pt}
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/frames_long.png}}}%
    \qquad
    \hspace{-25pt}
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/LDA_personachat_finetuned.png}}}%
    \qquad
    \hspace{-30pt}
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/tc_dailydialog.png}}}%
    \caption{From left to right, LDA downsampled representation of BERT on Frames (Goal oriented), MultiWOZ (Goal oriented), PersonaChat (chit-chat) and DailyDialog (chit-chat)}
    \vspace{-10pt}
    \label{fig:dialog_structure}
\end{figure*}

==> Unref Dialog Eval - ACL/sections/background.tex <==
We consider the problem of evaluating the response of a dialogue system, where an agent is provided with a sequence of sentences (or utterances) $c = \{u_1,u_2,...,u_n\}$ (termed as \textit{context}) to generate a \textit{response} $r=u_{n+1}$. Each utterance, $u_i$, can be represented as a set of words $u_i = \{w_1,w_2,...,w_n\}$. An utterance $u_i$ can be represented as a vector as $\vh_i = f_e(u_i)$, where $f_e$ is an encoder that encodes the words into a fixed vector representation. 

This work focuses on the evaluation of \textit{generative neural dialogue models}, which typically consist of an encoder-decoder style architecture that is trained to generate $u_{n+1}$ word-by-word \cite{serban2017hierarchical}.
The response of a generative model is typically evaluated by comparing with the ground-truth response using various automatic word-overlap metrics, such as BLEU or METEOR. These metrics, along with ADEM and RUBER, are essentially \textit{single-step} evaluation metrics, where a score is calculated for each context-response pair. If a dialogue $D_i$ contains $n$ utterances, we can extract $n-1$ context-response pairs : $(c_1  : \{u_1\}, r_1 : \{u_2\}), (c_2 : \{u_1, u_2\}, r_2 : \{u_3\}), \ldots, (c_{n-1} : \{u_1 \ldots u_{n-1}\}, r_{n-1} : u_n)$. In this paper, we are interested in devising a scalar metric that can evaluate the quality of a context-response pair: $\text{score}(c_i,r_i) = \mathcal{R} \in (0,1)$. 
A key benefit of this approach is that this metric can be used to evaluate online and also for better training and optimization, as it provides partial credit during response generation. 
%Recent research \cite{li2019acute, seeWhatMakesGood2019} although have shown the effectiveness of performing \textit{multi-step} human evaluations on dialogue, where an evaluator is shown the entire conversation $D_i = \{u_1, \ldots, u_n\}$ and asked to provide a rating, typically on the Likert scale. However, for an online setting, a multi-step evaluation leads to sparse rewards. In this work, we re-purpose single-step evaluation for online setting by proposing an unreferenced metric. This metric can be used to evaluate online and also for better training and optimization as it provides partial credit during response generation. 
%as compared to sparse rewards for multi-step evaluation. \comment{RL: do we argue this more in detail later? }
% This class of metrics is also known as \textit{referenced} metrics, as it requires the gold-truth response. However, these metrics are too restrictive as it doesn't account for semantic similarity, and as shown by \citet{liuHowNOTEvaluate2016}, they correlate poorly with human annotations.

%  There has been recent works in developing \textit{learned} dialogue evaluation metrics. \citet{loweAutomaticTuringTest2017a} propose ADEM, a referenced metric built to mimic human evaluations on the Ubuntu dialogue dataset. ADEM calculates a semantic similarity score between the context and response by comparison with the gold-truth response, and trains the model imitate human evaluations collected on the same dataset.
% \citet{taoRUBERUnsupervisedMethod2017} propose a hybrid referenced-unreferenced metric named RUBER, where the unreferenced metric is computed using negative sampling of random utterances from a different dialogue. 

% In essence, an \textit{unreferenced} metric is akin to computing semantic similarity between two sentences $(C,r)$. Computing the semantic similarity of two sentences is a growing field of research. \citet{wietingBLEUTrainingNeural2019} recently proposed the metric SIMILE, which is an unsupervised sentence similarity metric trained over large parallel corpus of paraphrased translations.

==> Unref Dialog Eval - ACL/sections/conclusion.tex <==
In this work, we explore the feasibility of learning an automatic dialogue evaluation metric by leveraging pre-trained language models and the temporal structure of dialogue. We propose \dtm{}, which is an unreferenced dialogue evaluation metric that leverages sentence representations from large pre-trained language models, and is trained via Noise Contrastive Estimation. \dtm{} also learns a recurrent neural network to model the transition between the utterances in a dialogue, allowing it to correlate better with human annotations. This is a good indication that \dtm{} can be used to evaluate online dialogue conversations. Since it provides immediate continuous rewards and at the single-step level, \dtm{} can be also be used to optimize and train better dialogue generation models, which we want to pursue as future work.

==> Unref Dialog Eval - ACL/sections/experiments.tex <==
To empirically evaluate our proposed unreferenced dialogue evaluation metric, we are interested in answering the following key research questions:

\begin{itemize}[itemsep=2pt, topsep=0pt]
    \item Q1: How robust is our proposed metric on different types of responses?
    \item Q2: How well does the self-supervised metric correlate with human judgements?
    % \item Q3: How well does the trained metric generalize on unseen data?
\end{itemize}

\xhdr{Datasets}  For training \dtm{}, we use PersonaChat \cite{zhang2018personalizing}, a large-scale open-domain chit-chat style dataset which is collected by human-human conversations over provided \textit{user persona}. We extract and process the dataset using ParlAI \cite{miller2017parlai} platform. We use the public train split for our training and validation, and the public validation split for testing. We use the human-human and human-model data collected by \citet{seeWhatMakesGood2019} for correlation analysis, where the models themselves are trained on PersonaChat.

% For analysis of dialogue structure, we use the goal oriented dataset Frames. Frames \cite{asri2017frames} is a restaurant booking dataset that provides information about a given dialogue state, to facilitate \emph{frame tracking}. We also use MultiWOZ \cite{budzianowski2018multiwoz} (goal-oriented) and DailyDialog \cite{li2017dailydialog} (chit-chat) for further analysis in Appendix \ref{sec:structure} and \ref{sec:generalization}.
%\comment{RL: maybe here also mention the See et al. data that you use for evaluation}
% We split all datasets in 80-20 split, where we report the scores on the held-out validation set.

\xhdr{Baselines} We use InferSent \cite{conneauSupervisedLearningUniversal2017} and unreferenced RUBER as  LSTM-based baselines. We also compare against BERT-NLI, which is the same as the InferSent model but with the LSTM encoder replaced with a pre-trained BERT encoder. 
Note that these baselines can be viewed as ablations of the \dtm{} framework using simplified text encoders, since we use the same NCE training loss to provide a fair comparison. 
Also, note that in practice, we use DistilBERT \cite{sanh2019distilbert} instead of BERT in both \dtm{} and the BERT-NLI baseline (and thus we refer to the BERT-NLI baseline as DistilBERT-NLI).\footnote{DistilBERT is the same BERT encoder with significantly reduced memory footprint and training time, which is trained by knowledge distillation \cite{buciluǎ2006model, hinton2015distilling} on the large pre-trained model of BERT.}.
%We fine-tune DistilBERT on PersonaChat dataset on masked language model objective before training our metric \footnote{The obvious choice of baseline would have been the unreferenced part of RUBER \cite{taoRUBERUnsupervisedMethod2017}. However, despite our best efforts, we were not able to get good results on PersonaChat dataset. In our experiments with RUBER, we found negligible difference in $\text{score}(c,r)$ and $\text{score}(c,\hat{r})$, which promted us to drop the baseline from consideration.}. All models are trained using Pytorch Lightning Framework \cite{Falcon2019}.
% We use subword units which is typically used in BERT-based models for all of our baselines to keep the evaluation fair.
%\comment{RL: I'd still add the RUBER results in the experiments, since the reviewers will probably ask about this. I think we've made a good-faith effort to reproduce it, and even asked the authors via email, etc.. We can even add this as another reason for proposing our metric in the introduction: we find that RUBER doesn't generalize well to the English-language datasets considered in this paper.}

\subsection{Evaluating \dtm{} on different types of responses}
\input{sections/model_ablations}

%\subsubsection{Effect of testing on different noise contrastive setups}

\subsection{Correlation with human judgements}
\input{sections/human_eval}



==> Unref Dialog Eval - ACL/sections/human_eval.tex <==
\label{sec:human_judgements}

%Evaluating the effectiveness of a metric is a chicken-and-egg problem : we cannot use yet another metric to evaluate the effectiveness of the proposed metric \comment{RL: don't think you need this sentence}. 
Metrics are evaluated on correlation with human judgements \cite{loweAutomaticTuringTest2017a, taoRUBERUnsupervisedMethod2017}, or by evaluating the responses of a generative model trained on the metric \cite{wietingBLEUTrainingNeural2019}, by human evaluation. However, this introduces a bias either during the questionnaire setup or during data post-processing in favor of the proposed metric. In this work, we refrain from collecting human annotations ourselves, but refer to the recent work by \citet{seeWhatMakesGood2019} on PersonaChat dataset. Thus, the evaluation of our metric is less subject to bias.

% \comment{RL: I don't fully understand this. why is correlation a biased metric? need more detail here, and some citations}. \ks{Hmm, I was kind of throwing this out in the air, but the thought process was that most papers report human annotation correlation by themselves and not a third party. This could potentially introduce a bias - be it in the questionnaire setup or data collection / cleaning. }

\citet{seeWhatMakesGood2019} conducted a large-scale human evaluation of 28 model configurations to study the effect of controllable attributes in dialogue generation. % In their evaluation, a crowdworker chats with either a model (model-human) or a human being (human-human, i.e. another crowdworker) in an online setting, and then answers a multiple choice question to capture 8 different aspects of conversation quality. These eight questions are Likert questions on a 1-4 scale, where higher is better. 
We use the publicly released model-human and human-human chat logs from \citet{seeWhatMakesGood2019} to generate the scores on our models, and correlate them with the associated human judgement on a Likert scale.
\citet{seeWhatMakesGood2019} propose to use a \textit{multi-step} evaluation methodology, where the human annotators rate the entire dialogue and not a context-response pair. On the other hand, our setup is essentially a \textit{single-step} evaluation method. To align our scores with the multi-turn evaluation, we average the individual turns to get an aggregate score for a given dialogue. 
\input{figures/human_uncalib}

\input{tab/calib_corr}

We investigate the correlation between the scores and uncalibrated individual human scores from 100 crowdworkers (Fig. \ref{fig:human_corr}), as well as aggregated scores released by \citet{seeWhatMakesGood2019} which are adjusted for annotator variance by using Bayesian calibration \cite{kulikov2018importance} (Table \ref{tab:human_corr_calib}). In all cases, we report Spearman's correlation coefficients.

For uncalibrated human judgements, we observe \dtm{} having higher relative correlation in 6 out of 8 quality measures. Interestingly, in case of calibrated human judgements, DistilBERT proves to be better in half of the quality measures. \dtm{} achieves marginally better overall correlation for calibrated human judgements, due to significantly strong correlation on specifically two measures: Interestingness and Engagingness. These measures answers the questions \textit{``How interesting or boring did you find this conversation?"} and \textit{``How much did you enjoy talking to this user?"}. (Refer to Appendix B of \citet{seeWhatMakesGood2019} for the full list of questions). Overall, using large pre-trained language models provides significant boost in the human correlation scores.

==> Unref Dialog Eval - ACL/sections/intro.tex <==
Recent approaches in deep neural language generation have opened new possibilities in dialogue generation \cite{serban2017hierarchical, weston2018retrieve}. Most of the current language generation efforts are centered around language modelling or machine translation \cite{ott2018scaling}, which are evaluated by comparing directly against the reference sentences. In dialogue, however, comparing with a single reference response is difficult, as there can be many reasonable responses given a context that have nothing to do with each other \cite{liuHowNOTEvaluate2016}. Still, dialogue research papers tend to report scores based on \textit{word-overlap} metrics from the machine translation literature (e.g. BLEU \cite{papineni2002bleu}, METEOR \cite{denkowski2014meteor}).  However word-overlap metrics aggressively penalize the generated response based on lexical differences with the ground truth and correlate poorly to human judgements \cite{liuHowNOTEvaluate2016}. 

\begin{figure}
    \centering
    \resizebox{0.5\textwidth}{!}{
    \includegraphics[]{figures/dialog_eval.png}}
    \caption{
   Model architecture for MaUdE, which is an unsupervised unreferenced metric for dialog evaluation.}
    \label{fig:worlds}
\end{figure}

%or in the summarization literature (ROUGE).

% \comment{RL: generating dialogue is a research area that existed before, so it didn't exactly get 'opened' by deep language generation. maybe 'has opened new possibilities in dialogue generation'? need a citation though}.
% \comment{RL: I'd switch gold truth -> reference. gold truth is like a mix of 'ground truth' and 'gold standard'}
% \comment{RL summarization? question answering?}

One can build dialogue evaluation metrics in two ways: \textit{referenced} metrics, which compare the generated response with a provided ground-truth response (such as the above word-overlap metrics), or an \textit{unreferenced} metrics, which evaluate the generated response without any such comparison. 
%also showed how such automatic metrics correlate poorly to human annotations - reinforcing the idea that word-overlap alone cannot judge the response quality accurately \comment{RL: unclear to me what this sentence means -- automatic metrics aren't just word overlap? also still seems to be saying the same thing}.
% However, a good dialogue response can have different lexical formations while maintaining semantic similarity with that of the ground truth \comment{RL: this is saying the same thing as the above paragraph}.
\citet{loweAutomaticTuringTest2017a} propose a \textit{learned referenced} metric named ADEM, which learns an alignment score between context and response to predict human score annotations. However, since the score is trained to mimic human judgements, it requires collecting large-scale human annotations on the dataset in question and cannot be easily applicable to new datasets \cite{loweRetrospectiveAutomaticTuring2019}.  
% \comment{RL: in my opinion, this is the most important point: learned reference metrics don't generalize well to other datasets / even within the same dataset (you can cite my retrospective: ml-retrospectives.github.io/published\_retrospectives/2019/adem/), and to create one with a new dataset you need to collect a lot of labels. I think this point should be emphasized more}. 

Recently, \citet{taoRUBERUnsupervisedMethod2017} proposed a hybrid referenced-unreferenced metric named RUBER, where the metric is trained without requiring human responses by bootstrapping negative samples directly from the dataset. 
%They report strong correlation with the human annotations on Chinese Douban corpus.
However, referenced metrics (including RUBER, as it is part referenced) are not feasible for evaluation of dialogue models in an \textit{online} setting---when the model is pitched against a human agent (model-human) or a model agent (model-model)---due to lack of a reference response. In this setting, models are usually evaluated directly by humans, which is costly and requires careful annotator training \cite{li2019acute}. 

The contributions of this paper are (1) a completely unsupervised unreferenced metric \dtm{} (\dtma{}), which leverages state-of-the-art pre-trained language models \cite{devlinBERTPretrainingDeep2018, sanh2019distilbert}, combined with a novel discourse-structure aware text encoder and contrastive training approach; and (2)
 results showing that \dtm{} has good correlation with human judgements.

% \comment{RL: I think the motivation for the 'unreferenced' part of the metric in the intro is a bit muddled and not entirely clear. It's super important for this to be clear, otherwise people won't believe the motivation and won't accept the paper. The current claims are something like: (1) just using a referenced metric 'overfits' too hard to the reference if you only have a single reference response (which usually you do), when in reality there are lots of different possible responses, (2) if you learn a referenced evaluation metric, it needs too much collected data, (3) if you combine referenced + unreferenced metrics (i.e. RUBER), then it's not feasible for evaluation dialogue models collected online. To me, points (1) and (2) make sense, but point (3) doesn't. Basically, right now we are trying hard to argue that using any information from the reference response is 'bad', but I think this is a losing battle (since the reference response *does* provide us useful information, it's just not all of the information we want). Instead, I think it would be best if we frame the paper as 'exploring the space of unreferenced metrics'. We can talk about why unreferenced metrics are important in general (because of reasons 1 and 2), and we can say that our analysis paves the way for better combinations of referenced + unreferenced metrics (maybe we can see if adding any referenced information --- e.g. BLEU / ROUGE score, or embedding based metrics --- improves our human correlation, if we have time before the deadline). }
%\ks{We are evaluating our proposed metrics on dialogue collected online - model to human or human to human conversations. My point was you cannot use a referenced metric here because you do not have any such reference or grounding of true response. We are not trying to argue adding reference response is bad in general, just that our use case doesn't allow us to do so.}
%\comment{rl: okay then, if that's the case that's great! but it has to be explained much better in the text, and more prominently. if referenced metrics aren't applicable here because it's online, that should be the first thing we talk about}

==> Unref Dialog Eval - ACL/sections/model.tex <==
\label{sec:model}

% We hypothesize that it is important for dialogue evaluation metrics to leverage the temporal structure of dialogue, since in dialogue the semantic representations of utterances follow a natural transition to the response. If we can effectively model this transition, then we may be able to leverage the dialogue conversation state to propose an effective metric. We analyze popular goal-oriented and chit-chat style datasets and observe that such temporal structure exists more clearly in the former (Figure \ref{fig:dialogue_structure_small}) For a detailed description of our analysis process, refer to Appendix \ref{sec:structure}. 

% \comment{RL: this is presented as a novel hypothesis, when in reality everyone who works on dialogue will agree with it and it's pretty obvious. instead, I'd say something like: "we hypothesize that it's important for dialogue evaluation metrics to leverage the temporal structure of dialogue". BLEU/ ROUGE/ word embedding methods don't really do this. you should also more specifically talk about how RUBER doesn't model temporal structure in a way that's 'good enough'}.
% \comment{RL: what do the colors mean? (I assume colored by turn). How does this show temporal structure / transitions?}.

% \input{figures/temporal_structure_two}

We propose a new model, \dtm{}, for online unreferenced dialogue evaluation. 
We first describe the general framework behind \dtm{}, which is inspired by the task of measuring alignment in natural language inference (NLI) \cite{williams2017broad}. It involves training text encoders via noise contrastive estimation (NCE) to distinguish between valid dialogue responses and carefully generated negative examples.
Following this, we introduce our novel text encoder that is designed to leverage the unique structural properties of dialogue. 

\dtm{} is designed to output a scalar $\text{score}(c_i,r_i) = \mathcal{R} \in (0,1)$, which measures how appropriate a response $r_i$ is given a dialogue context $c_i$.
This task is analogous to measuring alignment in NLI, but instead of measuring entailment or contradiction, our notion of alignment aims to quantify the \emph{quality} of a dialogue response.  
As in NLI, we approach this task by defining encoders $f_e^{\theta}(c)$ and $f_e^{\theta}(r)$ to encode the context and response, a combination function $f_{comb}(.)$ to combine the representations, and a final classifier $f_t(.)$, which outputs the alignment score:
\begin{equation}
\label{eq:setup}
    \text{score}(c,r) = \sigma(f_t(f_{comb}(f_e^{\theta_1}(c),f_e^{\theta_2}(r))).
\end{equation}

%Given that the task is to output a scalar $\text{score}(c_i,r_i) = \mathcal{R} \in (0,1)$, it can be viewed as a special case of finding alignment in natural language inference (NLI) \cite{williams2017broad}, where the output is the normalized probability of a binary classifier on entailment and contradiction. Concretely, we need encoders $f_e^{\theta}(c)$ and $f_e^{\theta}(r)$ to encode the context and response, a combination function $f_{comb}(.)$ to combine the representations, and a final classifier $f_t(.)$.



The key idea behind an unreferenced dialogue metric is the use of Noise Contrastive Estimation (NCE) \cite{gutmann2010noise} for training. Specifically, we train the model to differentiate between a correct response ($\text{score}(c,r) \to 1$), and a negative response ($\text{score}(c,\hat{r}) \to 0$), where $\hat{r}$ represents a candidate false response for the given context $c$. The loss to minimize contains one positive example and a range of negative examples chosen from a sampling policy $P(\hat{r})$:
\begin{equation}
    \mathcal{L} = - \log(\text{score}(c,r)) - \mathbb{E}_{\hat{r} \sim P(\hat{r})} \log ( - \text{score}(c,\hat{r})).
\end{equation}
\noindent The sampling policy $P(\hat{r})$ consists of \textit{syntactic} and \textit{semantic} negative samples. 

\xhdr{Syntactic negative samples} We consider three variants of syntax level adversarial samples: \textit{word-order} (shuffling the ordering of the words of $r$), \textit{word-drop} (dropping $x$\% of words in $r$) and \textit{word-repeat} (randomly repeating words in $r$).

\xhdr{Semantic negative samples} We also consider three variants of negative samples that are syntactically well formed, but represent corruption in the semantic space.  First, we choose a response $r_j$ which is chosen at random from a different dialogue such that $r_j \ne r_i$ (\textit{random utterance}). Second, we use a pre-trained seq2seq model on the dataset, and pair random seq2seq generated response with $r_i$ (\textit{random seq2seq}). Third, to provide a bigger variation of semantically negative samples, for each $r_i$ we generate high-quality paraphrases $r_i^b$ using Back-Translation \cite{edunov2018backtranslation}. We pair random Back-Translations $r_j^b$ with $r_i$ as in the above setup (\textit{random back-translation}). We also provide the paired $r_i^b$ as positive example for the models to learn variation in semantic similarity.
We further discuss the effect of different sampling policies in Appendix \ref{sec:nce}.

\xhdr{Dialogue-structure aware encoder}
Traditional NLI approaches (e.g., \citet{conneauSupervisedLearningUniversal2017}) use the general setup of Equation \ref{eq:setup} to score context-response pairs. The encoder $f_e$ is typically a Bidirectional LSTM---or, more recently, a BERT-based model \cite{devlinBERTPretrainingDeep2018}, which uses a large pre-trained language model. $f_{comb}$ is defined as in \citet{conneauSupervisedLearningUniversal2017}:
\begin{equation}
\label{eq:comb}
    f_{comb}(u,v) = \text{concat}([u,v,u*v,u-v]).
\end{equation} 
%Following the recent advancements of large pre-trained language models \cite{liu2019roberta}, we can also use an encoder $f_e$ that has more capacity and is (potentially) more powerful than an LSTM. 
%To this end, we use BERT \cite{devlinBERTPretrainingDeep2018} as an encoder to generate richer representations, keeping the rest of the setup as in Equation \ref{eq:setup} and $f_{comb}$ as in Equation \ref{eq:comb}. We call this model BERT-NLI. 
However, the standard text encoders used in these traditional NLI approaches ignore the temporal structure of dialogues, which is critical in our setting where the context is composed of a sequence of distinct utterances, with natural and stereotypical transitions between them. (See Appendix \ref{sec:structure} for a qualitative analysis of these transitions).
%Ideally, we would want to learn a \textit{transition function} which maps one utterance to the next. 
Thus we propose a specialized text encoder for \dtm{}, which uses a BERT-based encoder $f_e^{\text{BERT}}$ but additionally models dialogue transitions using a recurrent neural network:

%\comment{RL: another super important point: could the improvement just come from using BERT, vs. this whole 'learning a transition model' thing? I think this is a question that a reveiwer will definitely ask, so we should run that ablation if possible (i.e. try transition model + simple embedding, and BERT + not learning the transitions (maybe RUBER + BERT?). Update: seems like DistilBERT NLI is a decent baseline for this second one. }
%\ks{Ryan, I agree. However, the exact RUBER setting doesn't work at all for us. Hence, I used a BERT-based baseline (BERT-NLI) to show exactly the effect of using transition function :) }

%\input{figures/model_diagram.tex}

\begin{equation}
\label{eq:pool_eq}
\begin{split}
    \vh_{u_i} &= \mD_g f_e^{\text{BERT}}(u_i), \\
    \vh_{u_{i+1}}' &= f_R(\vh_{u_i}, \vh_{u_i}'), \\
    \vc_i &= \mW.\text{pool}_{\forall t \in \{u_1,\ldots,u_{n-1}\}}(\vh_{t}') \\
    \text{score}(c_i,r_i) &= \sigma (f_{t} ([\vh_{r_i}, \vc_{i}, \vh_{r_i}*\vc_i, \vh_{r_i}-\vc_{i}])),
\end{split}
\end{equation}

\noindent where $\vh_{u_i} \in \mathcal{R}^d$ is a downsampled BERT representation of the utterance $u_i$ (using a global learned mapping $\mD_g \in \mathcal{R}^{B\times d}$).  $\vh_{u_i}'$ is the hidden representation of $f_R$ for $u_i$, where $f_R$ is a Bidirectional LSTM.
The final representation of the dialogue context is learned by pooling the individual hidden states of the RNN using max-pool (Equation \ref{eq:pool_eq}). This context representation is mapped into the response vector space using weight $\mW$, to obtain $\vc_i$. We then learn the alignment score between the context $\vc_i$ and response $r_i$'s representation $\vh_{r_i}$ following Equation \ref{eq:setup}, by using the combination function $f_{comb}$ being the same as in Equation \ref{eq:comb}.

% \xhdr{Training} In order to train the $\text{score}(c,r)$ in a self-supervised way from the dataset itself, we consider the standard Noise Contrastive Estimation (NCE) setting \cite{gutmann2010noise}. The loss to minimize contains the \textit{true score}, i.e $\text{score}(c,r)$ and a set of \textit{negative scores}, i.e  $\text{score}(c,\hat{r})$, where $\hat{r}$ represents a candidate false response for the given context $c$. This loss trains the parameters for $f_e, f_R, \mD$ and $\mW$ end-to-end.



==> Unref Dialog Eval - ACL/sections/model_ablations.tex <==
\label{sec:ablations}

We first analyze the robustness of \dtm{} by comparing with the baselines, by using the same NCE training for \textit{all the models} for fairness. We evaluate the models on the \textit{difference} score, $\Delta = \text{score}(c,r_{\text{ground-truth}}) - \text{score}(c,r)$ (Table \ref{tab:ablation}). $\Delta$ provides an insight on the range of score function. An optimal metric would cover the full range of good and bad responses. We evaluate response $r$ in three settings: \textit{Semantic Positive}: responses that are semantically equivalent to the ground truth response; \textit{Semantic Negative}: responses that are semantically opposite to the ground truth response; and \textit{Syntactic Negative}: responses that have been adversarially modified in the lexical units.  Ideally, we would want $\Delta \to 1$ for semantic and syntactic negative responses, $\Delta \to 0$ for semantic positive responses. 

\input{tab/ablation_short}

%evaluated on the held-out test set of PersonaChat dataset \footnote{The public release of PersonaChat dataset contains training and validation files, but not the test set. We use the validation set as our test set, while we split the training set 80-20 for internal validation.}. 

% \footnote{Although this enforces a strong assumption that a trained seq2seq model provides semantically equivalent responses, which might not be the case. We refrained from training seq2seq examples as either as positive or negative datapoints in our NCE setup precisely due to this reason. Instead, we use random seq2seq responses as negative examples which are more consistent with our intuition.}
%\comment{RL: I don't quite understand the above sentences}

%\comment{RL: I find Table 1, in it's current form, to be confusing (it's important that, if you look at the table, it makes sense without too much effort :D). is higher better, or is lower better? why does infersent have so many bold scores (which indicates the best scores?). is the 'score' or the 'delta' more important? ideally we wouldn't separate based on 'semantic positive', 'semantic negative', etc., and we'd just have 1 main table with the overall results (and maybe have the bigger table in the appendix).}

We observe that the \dtm{} scores perform robustly across all the setups. RUBER and InferSent baselines are weak, quite understandably so because they cannot leverage the large pre-trained language model data and thus is poor at generalization. DistilBERT-NLI baseline performs significantly better than InferSent and RUBER, while \dtm{} scores even better and more consistently overall. We provide a detailed ablation of various training scenarios as well as the absolute raw $\Delta$ scores in Appendix \ref{sec:nce}. We also observe both \dtm{} and DistilBERT-NLI to be more robust on zero-shot generalization to different datasets, the results of which are available in Appendix \ref{sec:generalization}.

==> Unref Dialog Eval - ACL/tab/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|ll|ll|ll|ll|}
\hline
PersonaChat Dataset & Model & \multicolumn{2}{c}{RUBER} & \multicolumn{2}{c|}{InferSent} & \multicolumn{2}{c|}{DistilBERT NLI} & \multicolumn{2}{c|}{\dtm{}} \\ \cline{2-10} 
 & Training Modes & \multicolumn{2}{c}{All} & \multicolumn{2}{c|}{All} & \multicolumn{2}{c|}{All} & \multicolumn{2}{c|}{All} \\ \cline{2-10} 
 & Evaluation Modes & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ \\ \hline
\multirow{3}{*}{Semantic Positive} & Gold Truth Response & 0.432\tiny$\pm{0.213}$ & 0 & 0.462\tiny$\pm{0.254}$ & 0 & 0.824\tiny$\pm{0.154}$ & 0 & \textbf{0.909}\tiny$\pm{0.152}$ & 0 \\
 & BackTranslation & 0.183\tiny$\pm{0.198}$ & 0.249 & 0.184\tiny$\pm{0.218}$ & 0.278 & 0.8\tiny$\pm{0.19}$ & \boldblue{0.024} & \textbf{0.838}\tiny$\pm{0.227}$ & 0.070 \\
 & Seq2Seq & 0.09\tiny$\pm{0.17}$ & 0.342 & 0.10\tiny$\pm{0.184}$ & 0.362 & \textbf{0.65}\tiny$\pm{0.287}$ & \boldblue{0.174} & 0.6008\tiny$\pm{0.38}$ & 0.308 \\ \hline
\multirow{2}{*}{Semantic Negative} & Random Utterance & 0.28\tiny$\pm{0.21}$ & 0.152 & \textbf{0.252}\tiny$\pm{0.236}$ & 0.209 & 0.677\tiny$\pm{0.255}$ & 0.147 & 0.621\tiny$\pm{0.344}$ & \boldblue{0.287} \\
 & Random Seq2Seq & 0.03\tiny$\pm{0.09}$ & 0.402 & \textbf{0.026}\tiny$\pm{0.079}$ & 0.435 & 0.48\tiny$\pm{0.313}$ & 0.344 & 0.323\tiny$\pm{0.355}$ & \boldblue{0.585} \\ \hline 
\multirow{3}{*}{Syntactic Negative} & Word Drop & \textbf{0.09}\tiny$\pm{0.16}$ & 0.342 & 0.094\tiny$\pm{0.17}$ & \boldblue{0.367} & 0.563\tiny$\pm{0.377}$ & 0.261 & 0.609\tiny$\pm{0.401}$ & 0.3 \\
 & Word Order & \textbf{0.04}\tiny$\pm{0.10}$ & 0.392 & 0.052\tiny$\pm{0.112}$ & 0.409 & 0.153\tiny$\pm{0.29}$ & 0.671 & 0.182\tiny$\pm{0.327}$ & \boldblue{0.726} \\
 & Word Repeat & \textbf{0.00}\tiny$\pm{0.01}$ & 0.432 & 0.001\tiny$\pm{0.010}$ & 0.461 & 0.041\tiny$\pm{0.153}$ & 0.782 & 0.036\tiny$\pm{0.151}$ & \boldblue{0.872} \\ \hline
\end{tabular}%%
}
\caption{Metric score evaluation between InferSent, DistilBERT-NLI and \dtm{} on PersonaChat dataset, trained on $P(\hat{r})$ = Syntax + Semantics. Bold scores represent the best individual scores, and bold with blue represents the best difference with the true response.}
\label{tab:ablation}
\end{table*}

==> Unref Dialog Eval - ACL/tab/ablation_semantics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|ll|ll|ll|ll|}
\hline
PersonaChat Dataset & Model & \multicolumn{2}{c|}{RUBER} & \multicolumn{2}{c|}{InferSent} & \multicolumn{2}{c|}{DistilBERT NLI} & \multicolumn{2}{c|}{\dtm{}} \\ \cline{2-10} 
 & Training Modes & \multicolumn{2}{c|}{Only Semantics} & \multicolumn{2}{c|}{Only Semantics} & \multicolumn{2}{c|}{Only Semantics} & \multicolumn{2}{c|}{Only Semantics} \\ \cline{2-10} 
 & Evaluation Modes & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ \\ \hline
\multirow{3}{*}{Semantic Positive} & Gold Truth Response & 0.443\tiny$\pm{0.197}$ & 0 & 0.466\tiny$\pm{0.215}$ & 0 & 0.746\tiny$\pm{0.236}$ & 0 & \textbf{0.789}\tiny$\pm{0.244}$ & 0 \\
 & BackTranslation & 0.296\tiny$\pm{0.198}$ & 0.147 & 0.273\tiny$\pm{0.195}$ & 0.192 & \textbf{0.766}\tiny$\pm{0.235}$ & -0.02 & 0.723\tiny$\pm{0.277}$ & \boldblue{0.066} \\
 & Seq2Seq & 0.082\tiny$\pm{0.163}$ & 0.361 & 0.10\tiny$\pm{0.184}$ & 0.367 & \textbf{0.46}\tiny$\pm{0.357}$ & \boldblue{0.286} & 0.428\tiny$\pm{0.390}$ & 0.361 \\ \hline
\multirow{2}{*}{Semantic Negative} & Random Utterance & 0.299\tiny$\pm{0.203}$ & 0.144 & \textbf{0.287}\tiny$\pm{0.208}$ & 0.178 & 0.489\tiny$\pm{0.306}$ & 0.257 & 0.388\tiny$\pm{0.335}$ & \boldblue{0.40} \\
 & Random Seq2Seq & \textbf{0.028}\tiny$\pm{0.077}$ & 0.415 & 0.036\tiny$\pm{0.082}$ & 0.429 & 0.237\tiny$\pm{0.283}$ & 0.529 & 0.16\tiny$\pm{0.26}$ & \boldblue{0.629} \\ \hline 
\multirow{3}{*}{Syntactic Negative} & Word Drop & 0.334\tiny$\pm{0.206}$ & 0.109 & \textbf{0.308}\tiny$\pm{0.217}$ & \boldblue{0.158} & 0.802\tiny$\pm{0.224}$ & -0.056 & 0.73\tiny$\pm{0.29}$ & 0.059 \\
 & Word Order & \textbf{0.472}\tiny$\pm{0.169}$ & -0.029 & 0.482\tiny$\pm{0.19}$ & -0.016 & 0.685\tiny$\pm{0.284}$ & 0.061 & 0.58\tiny$\pm{0.35}$ & \boldblue{0.209} \\
 & Word Repeat & 0.255\tiny$\pm{0.24}$ & 0.188 & \textbf{0.153}\tiny$\pm{0.198}$ & 0.312 & 0.657\tiny$\pm{0.331}$ & 0.089 & 0.44\tiny$\pm{0.39}$ & \boldblue{0.349} \\ \hline
\end{tabular}%
}
\caption{Metric score evaluation between InferSent, DistilBERT-NLI and \dtm{} on PersonaChat dataset, trained on $P(\hat{r})$ = Semantics. Bold scores represent the best individual scores, and bold with blue represents the best difference with the true response.}
\label{tab:ablation_semantics}
\end{table*}

==> Unref Dialog Eval - ACL/tab/ablation_short.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|lllll|}
\hline
                                    &            & R & IS      & DNLI & M         \\ \hline
Semantic Positive $\downarrow$                   & BackTranslation  & 0.249 & 0.278          & \textbf{0.024} & 0.070          \\
                                    & Seq2Seq          & 0.342 & 0.362          & \textbf{0.174} & 0.308          \\ \hline
\multirow{2}{*}{Semantic Negative $\uparrow$}  & Random Utterance & 0.152 & 0.209          & 0.147          & \textbf{0.287} \\
                                    & Random Seq2Seq   & 0.402 & 0.435          & 0.344          & \textbf{0.585} \\ \hline
\multirow{3}{*}{Syntactic Negative $\uparrow$} & Word Drop        & 0.342 & \textbf{0.367} & 0.261          & 0.3            \\
                                    & Word Order       & 0.392 & 0.409          & 0.671          & \textbf{0.726} \\
                                    & Word Repeat      & 0.432 & 0.461          & 0.782          & \textbf{0.872} \\ \hline
\end{tabular}%
}
\caption{\small{Metric score evaluation ($\Delta = \text{score}(c,r_{\text{ground-truth}}) - \text{score}(c,r)$) between RUBER (R), InferSent (IS), DistilBERT-NLI (DNI) and \dtm{} (M) on PersonaChat dataset's public validation set. For Semantic Positive tests, lower $\Delta$ is better; for all Negative tests higher $\Delta$ is better.}}
\label{tab:ablation_short}
\end{table}

==> Unref Dialog Eval - ACL/tab/ablation_syntax.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|ll|ll|ll|ll|}
\hline
PersonaChat Dataset & Model & \multicolumn{2}{c|}{RUBER} & \multicolumn{2}{c|}{InferSent} & \multicolumn{2}{c|}{DistilBERT NLI} & \multicolumn{2}{c|}{\dtm{}} \\ \cline{2-10} 
 & Training Modes & \multicolumn{2}{c|}{Only Syntax} & \multicolumn{2}{c|}{Only Syntax} & \multicolumn{2}{c|}{Only Syntax} & \multicolumn{2}{c|}{Only Syntax} \\ \cline{2-10} 
 & Evaluation Modes & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ & \multicolumn{1}{l|}{Score} & $\Delta$ \\ \hline
\multirow{3}{*}{Semantic Positive} & Gold Truth Response & 0.891\tiny$\pm{0.225}$ & 0 & 0.893\tiny$\pm{0.231}$ & 0 & 0.986\tiny$\pm{0.088}$ & 0 & \textbf{0.99}\tiny$\pm{0.07}$ & 0 \\
 & BackTranslation & 0.687\tiny$\pm{0.363}$ & 0.204 & 0.672\tiny$\pm{0.387}$ & 0.221 & 0.877\tiny$\pm{0.268}$ & 0.109 & \textbf{0.91}\tiny$\pm{0.23}$ & \boldblue{0.08} \\
 & Seq2Seq & 0.929\tiny$\pm{0.187}$ & -0.038 & 0.949\tiny$\pm{0.146}$ & -0.055 & 0.996\tiny$\pm{0.048}$ & -0.01 & \textbf{0.99}\tiny$\pm{0.05}$ & \boldblue{0.00} \\ \hline
\multirow{2}{*}{Semantic Negative} & Random Utterance & 0.869\tiny$\pm{0.248}$ & 0.022 & \textbf{0.835}\tiny$\pm{0.294}$ & \boldblue{0.058} & 0.977\tiny$\pm{0.116}$ & 0.009 & 0.97\tiny$\pm{0.13}$ & 0.02 \\
 & Random Seq2Seq & 0.915\tiny$\pm{0.196}$ & -0.024 & \textbf{0.904}\tiny$\pm{0.206}$ & -0.011 & 0.994\tiny$\pm{0.057}$ & -0.008 & 0.99\tiny$\pm{0.08}$ & \boldblue{0} \\ \hline
\multirow{3}{*}{Syntactic Negative} & Word Drop & 0.119\tiny$\pm{0.255}$ & 0.772 & \textbf{0.105}\tiny$\pm{0.243}$ & \boldblue{0.788} & 0.373\tiny$\pm{0.414}$ & 0.613 & 0.41\tiny$\pm{0.44}$ & 0.584 \\
 & Word Order & 0.021\tiny$\pm{0.101}$ & 0.87 & \textbf{0.015}\tiny$\pm{0.0915}$ & 0.878 & 0.064\tiny$\pm{0.194}$ & 0.922 & 0.07\tiny$\pm{0.21}$ & \boldblue{0.928} \\
 & Word Repeat & \textbf{0.001}\tiny$\pm{0.007}$ & 0.89 & \textbf{0.001}\tiny$\pm{0.020}$ & 0.893 & 0.006\tiny$\pm{0.057}$ & 0.980 & 0.01\tiny$\pm{0.06}$ & \boldblue{0.981} \\ \hline
\end{tabular}%
}
\caption{Metric score evaluation between InferSent, DistilBERT-NLI and \dtm{} on PersonaChat dataset, trained on $P(\hat{r})$ = Syntax. Bold scores represent the best individual scores, and bold with blue represents the best difference with the true response.}
\label{tab:ablation_syntax}
\end{table*}

==> Unref Dialog Eval - ACL/tab/calib_corr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
                    & R          & IS & DNLI & M         \\ \cline{2-5} 
Fluency             & 0.322          & 0.246     & \textbf{0.443} & 0.37           \\
Engagingness        & 0.204          & 0.091     & 0.192          & \textbf{0.232} \\
Humanness           & 0.057          & -0.108    & \textbf{0.129} & 0.095          \\
Making Sense        & 0.0            & 0.005     & \textbf{0.256} & 0.208          \\
Inquisitiveness     & 0.583          & 0.589     & 0.598          & \textbf{0.728} \\
Interestingness     & \textbf{0.275} & 0.119     & 0.135          & 0.24           \\
Avoiding Repetition & \textbf{0.093} & -0.118    & -0.039         & -0.035         \\
Listening           & 0.061          & -0.086    & \textbf{0.124} & 0.112          \\ \hline
Mean                & 0.199          & 0.092     & 0.23           & \textbf{0.244} \\ \hline
\end{tabular}%
}
\caption{\small{Correlation with calibrated scores between RUBER (R), InferSent (IS), DistilBERT-NLI (DNI) and \dtm{} (M) when trained on PersonaChat dataset}}
\label{tab:human_corr_calib}
\vspace{-2mm}
\end{table}

==> Unref Dialog Eval - ACL/tab/zero_shot.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ccl|ll|ll|}
\hline
Datasets & \multicolumn{1}{l|}{} & \multicolumn{2}{l|}{DailyDialog} & \multicolumn{2}{l|}{Frames} & \multicolumn{2}{l|}{MultiWOZ} \\ \hline
Model & \multicolumn{1}{c}{Eval Mode} & \multicolumn{1}{c}{Score} & $\Delta$ & \multicolumn{1}{l}{Score} & $\Delta$ & \multicolumn{1}{l}{Score} & $\Delta$ \\ \hline
\multirow{2}{*}{RUBER} 
& $+$ & 0.173 $\pm{0.168}$ &  & 0.211 $\pm{0.172}$ &  & 0.253 $\pm{0.177}$ &  \\
 & $-$ & 0.063 $\pm{0.092}$ & 0.11 & 0.102 $\pm{0.114}$ & 0.109 & 0.121 $\pm{0.123}$ & 0.123 \\ \hline
\multirow{2}{*}{InferSent} 
& $+$ & 0.163 $\pm{0.184}$ &  & 0.215 $\pm{0.186}$ &  & 0.277 $\pm{0.200}$ &  \\
 & $-$ & 0.050 $\pm{0.085}$ & 0.113 & 0.109 $\pm{0.128}$ & 0.106 & 0.127 $\pm{0.133}$ & 0.15 \\ \hline
\multirow{2}{*}{DistilBERT NLI} 
& $+$ & 0.885 $\pm{0.166}$ &  & 0.744 $\pm{0.203}$ &  & 0.840 $\pm{0.189}$ &  \\
 & $-$ & 0.575 $\pm{0.316}$ & 0.31 & 0.538 $\pm{0.330}$ & 0.206 & 0.566 $\pm{0.333}$ & 0.274 \\ \hline
\multirow{2}{*}{\dtm{}}
& $+$ & 0.782 $\pm{0.248}$ &  & 0.661 $\pm{0.293}$ &  & 0.758 $\pm{0.265}$ & \\ 
& $-$ & 0.431 $\pm{0.300}$ & \textbf{0.351} & 0.454 $\pm{0.358}$ & \textbf{0.207} & 0.483 $\pm{0.345}$ & \textbf{0.275} \\ \hline
\end{tabular}%
}
\caption{Zero-shot generalization results on DailyDialog, Frames and MultiWOZ dataset for the baselines and \dtm{}. $+$ denotes semantic positive responses, and $-$ denotes semantic negative responses.}
\label{tab:zero_shot}
\end{table*}

==> figures/model_diagram.tex <==
\begin{figure}[htb]
\centering
%\resizebox{0.5\textwidth}{!}{\includegraphics[]{figures/model_diag_desc.jpeg}}
%\resizebox{0.5\textwidth}{!}{\input{figures/model_diagram.tikz}}
\caption{Model diagram of \dtm{}}\label{fig:model_diagram}
\end{figure}

==> figures/temporal_structure_two.tex <==
\begin{figure}[!htb]
     \centering
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/frames_short.png}}}%
    \qquad
    \hspace{-27pt}
    \subfloat{{\includegraphics[width=0.24\textwidth]{figures/LDA_personachat_finetuned.png}}}%
    \caption{LDA downsampled representation of BERT on Frames (Goal oriented), and PersonaChat (chit-chat). The clusters denote the binning of each utterance, where purple denotes the first bin and red denotes the last bin.}
    \vspace{-10pt}
    \label{fig:dialog_structure_small}
\end{figure}
